Investigating the Benefits of Free-Form Rationales

Free-form rationales aim to aid model interpretability by supplying the background knowledge that can help understand model decisions. Crowdsourced rationales are provided for commonsense QA instances in popular datasets such as CoS-E and ECQA, but their utility remains under-investigated. We present human studies which show that ECQA rationales indeed provide additional background information to understand a decision, while over 88% of CoS-E rationales do not. Inspired by this finding, we ask: can the additional context provided by free-form rationales benefit models, similar to human users? We investigate the utility of rationales as an additional source of supervision, by varying the quantity and quality of rationales during training. After controlling for instances where rationales leak the correct answer while not providing additional background knowledge, we find that incorporating only 5% of rationales during training can boost model performance by 47.22% for CoS-E and 57.14% for ECQA during inference. Moreover, we also show that rationale quality matters: compared to crowdsourced rationales, T5-generated rationales provide not only weaker supervision to models, but are also not helpful for humans in aiding model interpretability.

==> content/arxiv-4-1.tex <==
\input{tables/1-difficulty}

% We first conduct experiments to understand how hard it is for machines to solve the commonsense question answering task. 

As a first empirical investigation, we use rationales from \cose v1.0 and \cose v1.11 as additional supervision to task models, following the IR$\rightarrow$O set up, as defined in \S\ref{sec:tasks}.
% Therefore, we start with them to justify our modeling choice and establish a benchmark for future analysis. 
% First, we use the complete set of rationale annotation during both model training and inference time.
As a baseline, we use the I$\rightarrow$O set up, which does not have access to any rationales at either train or test time.
We consider three models: UnifiedQA~\cite{khashabi-etal-2020-unifiedqa} in a zero-shot setting, as well as UnifiedQA\footnote{
We use released models and instructions for finetuning from \url{https://github.com/allenai/unifiedqa}.} and T5 \cite{t5}, finetuned on the respective \cose benchmarks.
We choose UnifiedQA, a state-of-the-art T5-based question answering model, because it not only performs well across twenty QA datasets, but also shows great generalization to out-of-domain data.

Our results in Table~\ref{tab:difficulty} show that under each setting, using crowdsourced rationales both during training and inference greatly improves model performance, even under a zero-shot setting.
With finetuning, T5-base performs comparably to UnifiedQA.\footnote{This justifies our choice of T5 for later experiments. Additionally, given the higher difficulty of the \cose v1.11 task (5 answer choices, vs. 3 in v1.0), we use \cose v1.11 for the rest of our analysis.}
Most remarkably, \ecqa performance is almost perfect after including rationales during finetuning.
However, as our human study in \S\ref{sec:human} suggested, the improvement may come from the direct leakage of the correct answers. 
Thus, we next investigate workarounds to address the leakage problem in \cose and \ecqa.

==> tables/0-statistics.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{@{}llr@{}}
\toprule
\textbf{Dataset} & \textbf{Train} & \textbf{Test} \\ \midrule
% \cose v1.0        & 7,610          & 950           \\
\cose v1.11/\ecqa  & 9,741          & 1,221         \\
\quartz           & 2,695          & 783           \\ \bottomrule
\end{tabular}
\vspace{-0.1mm}
\caption{The statistics of 3 datasets in our work.
\vspace{-0.3cm}
\swabha{consider moving the table to appendix to save space.}}
\label{tab:statistics}
\end{table}

==> tables/1-difficulty.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\small
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule
   & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ UnifiedQA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Finetuned \\ UnifiedQA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Finetuned\\ T5\end{tabular}} \\ \midrule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}CoS-E \\ v1.0\end{tabular}} & 
I$\rightarrow$O & 60\% & \textbf{66\%} & 65\% \\
IR$_\textrm{\cose v1.0}\rightarrow$O & 70\% & 88\% & \textbf{89\%} \\ 
\midrule[0.01em]
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}CoS-E \\ v1.11\end{tabular}} & 
I$\rightarrow$O & 45\% & \textbf{56\%} & \textbf{56\%} \\
IR$_\textrm{\cose v1.1}\rightarrow$O & 54\% & 76\% & \textbf{78\%} \\
IR$_\textrm{\ecqa}\rightarrow$O & 86\% & \textbf{98\%}  & \textbf{98\%}\\
\bottomrule
\end{tabular}
}
\caption{
Model accuracy improves with rationales from \cose v1.0, \cose v1.11 and \ecqa as additional supervision signals. 
We see great improvements under both a zero-shot setting with UnifiedQA, as well as after finetuning UnifiedQA and T5.
% We use CoS-E v1.0 and CoS-E v1.11 to estimate how difficult the common sense task is with prediction accuracy. 
% For our experiment, we considered three types of models: pre-trained UnifiedQA (base)~\cite{khashabi-etal-2020-unifiedqa}, finetuned UnifiedQA (base) and finetuned T5 (base) model. 
% Finetuned T5 model achieves comparable performances with finetuned UnifiedQA models. 
All rationales $R$ here are from crowdsourcing, hence based on the gold label.}
\label{tab:difficulty}
\vspace{-2mm}
\end{table}

